Physics-Free Spectrally Multiplexed Photometric Stereo under Unknown Spectral Composition

In this paper, we present a groundbreaking spectrally multiplexed photometric stereo approach for recovering surface normals of dynamic surfaces without the need for calibrated lighting or sensors, a notable advancement in the field traditionally hindered by stringent prerequisites and spectral ambiguity. By embracing spectral ambiguity as an advantage, our technique enables the generation of training data without specialized multispectral rendering frameworks. We introduce a unique, physics-free network architecture, SpectraM-PS, that effectively processes multiplexed images to determine surface normals across a wide range of conditions and material types, without relying on specific physically-based knowledge. Additionally, we establish the first benchmark dataset, SpectraM14, for spectrally multiplexed photometric stereo, facilitating comprehensive evaluations against existing calibrated methods. Our contributions significantly enhance the capabilities for dynamic surface recovery, particularly in uncalibrated setups, marking a pivotal step forward in the application of photometric stereo across various domains.

==> sec/4_universal_mps.tex <==
\section{Universal Multispectral Photometric Stereo}
\label{sec:unimps}
\begin{figure}[t]
	\begin{center}
		\includegraphics[width=85mm]{figures/multiplexing.pdf}
	\end{center}
	\vspace{-10pt}
	\caption{(upper) Illustration of calibrated multispectral photometric stereo: This figure depicts a setup with a known single directional light source. It also demonstrates the alignment of sensor spectral sensitivity with the spectral distribution of the light source, ensuring no crosstalk. (lower) Depiction of universal multispectral photometric stereo: This figure represents a scenario where the number and spatial distribution of light sources are unknown. It also illustrates the potential mismatch between sensor spectral sensitivity and light source spectral distribution, which may lead to crosstalk.}
	\vspace{-10pt}
	\label{fig:multispectral}
\end{figure}
Multispectral Photometric Stereo (MPS) aims to recover a normal map $N\in \mathbb{R}^{H\times W \times 3}$ from single-channel images $I_k\in \mathbb{R}^{H\times W}$, captured under $K$ distinct lighting conditions. These lighting conditions have varying spatial and spectral distributions, and the images are obtained using fixed, orthographic sensors with diverse spectral responses. To assist in the reconstruction process, an optional object mask $M\in \mathbb{R}^{H\times W}$ may also be utilized.

As delineated in~\cref{fig:multispectral} (upper), we introduce the concept of Universal Multispectral Photometric Stereo, a sophisticated process aiming to reconstruct the surface map of an object from multispectral images, which is characterized by a set of intricate unknowns:
\begin{enumerate}
\item The spatial and spectral distributions of the illuminating light sources are indeterminate.
\item The spectral sensitivity profile of the imaging sensor is unspecified.
\item There is an inherent risk of spectral crosstalk among the imaging channels.
\end{enumerate}
This definition highlights the flexibility and adaptability of universal MPS in handling diverse and uncontrolled environments, distinguishing it from traditional, calibrated MPS methods that demands a setup with a single-directional, precisely calibrated light source and a specialized camera system that minimizes crosstalk between spectral bands as illustrated in~\cref{fig:multispectral} (lower). This flexibility broaden its applicability in real-world scenarios where strict lighting control and specialized equipment are not feasible.
